A Simple and Efficient Baseline for Data Attribution on Images

Data attribution methods play a crucial role in understanding machine learning models, providing insight into which training data points are most responsible for model outputs during deployment. However, current state-of-the-art approaches require a large ensemble of as many as 300,000 models to accurately attribute model predictions. These approaches therefore come at a high computational cost, are memory intensive, and are hard to scale to large models or datasets. In this work, we focus on a minimalist baseline, utilizing the feature space of a backbone pretrained via self-supervised learning to perform data attribution. Our method is model-agnostic and scales easily to large datasets. We show results on CIFAR-10 and ImageNet, achieving strong performance that rivals or outperforms state-of-the-art approaches at a fraction of the compute or memory cost. Contrary to prior work, our results reinforce the intuition that a model's prediction on one image is most impacted by visually similar training samples. Our approach serves as a simple and efficient baseline for data attribution on images.

==> figures/joint_k_leave_out_imagenet_and_lds_score_cifar10.tex <==
\begin{figure}
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \input{figures/k_leave_out_imagenet}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \input{tables/lds_scores}
        \vspace{1.41cm}
    \end{minipage}
    \par
    \vspace{-0.5cm}
    \begin{minipage}[t]{0.45\textwidth}
        \caption{\textbf{Our method yields better upper bounds on support size compared to TRAK-4, which requires more storage than the ImageNet dataset itself.} We estimate data removal support for 30 random ImageNet validation samples and plot the CDF of estimates.}
        \label{fig:k-leave-out-imagenet}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.45\textwidth}
        \captionof{table}{We compare LDS scores for our approach with other baselines on CIFAR-10. Our proposed approach can perform equivalent to TRAK with $5$ models.}
        \label{tab:lds-scores}
    \end{minipage}
\end{figure}

==> sections/motivation.tex <==


\section{The Role of Data Attribution}
\label{sec:motivation}

In various real-world machine learning systems, for healthcare or finance, we often seek to answer questions like, ``Which samples of the input data influenced this prediction?" or ``How sensitive is this model prediction to changes in the training data?". These counterfactual insights enable us to assess the impact of hypothetical changes in the data distribution, which in turn help us understand  the basis of the model's decisions, and how to change the decision in the event of an error.

 Consider the scenario where we desire to understand how a model's prediction would change if a specific data point were altered or removed. The naive solution to this problem involves retraining the model after modifying the dataset, which quickly becomes intractable beyond small models and modest dataset sizes. Data attribution approaches aim to provide a more computationally feasible solution to this problem. However, this leads to a trade-off for different data attribution methods between computational efficiency and performance. 

% A primary motivation for data attribution lies in counterfactual estimation. These approaches aim to provide computationally feasible solutions to perform counterfactual estimation. 
Influence functions and it's approximations \citep{koh2017understanding, } the first to provide a computationally attractive solution

% focus on data provenance in introduction, and counterfactual is a way of formalizing this.

% accurate, cheap and scalable.

% As machine learning systems become more prevalent, there's a rising need for understanding their behaviour. This has lead to critical questions surrounding these models, such as: ``Why did the model make this specific prediction?'' ``What aspects of input data influenced this prediction?'' To formalize this question, \citep{koh2017understanding} 

==> sections/reproducibility.tex <==
\section{Reproducibility}

For reproducibility, our supplementary material includes the source code and top-k training indexes from baselines and our method. We will also release the model weights, but these are too large to include in the supplementary. We also discuss our full experimental setup and include links to the baselines we used in \Cref{sec:experimental-setup}. Details regarding our evaluation metrics are described in \Cref{sec:methodology} and \Cref{app:compute-description}. Our experiments utilize randomly selected validation samples from CIFAR-10 \citep{krizhevsky2009learning} and Imagenet \citep{deng2009imagenet}, and we also include indices for these validation samples with our supplementary material.
